Flight: A FaaS-Based Framework for Complex and Hierarchical Federated Learning

Federated Learning (FL) is a decentralized machine learning paradigm where models are trained on distributed devices and are aggregated at a central server. Existing FL frameworks assume simple two-tier network topologies where end devices are directly connected to the aggregation server. While this is a practical mental model, it does not exploit the inherent topology of real-world distributed systems like the Internet-of-Things. We present Flight, a novel FL framework that supports complex hierarchical multi-tier topologies, asynchronous aggregation, and decouples the control plane from the data plane. We compare the performance of Flight against Flower, a state-of-the-art FL framework. Our results show that Flight scales beyond Flower, supporting up to 2048 simultaneous devices, and reduces FL makespan across several models. Finally, we show that Flight's hierarchical FL model can reduce communication overheads by more than 60%.

==> code-snippets/worker_strategy.tex <==
\begin{lstlisting}[
    caption={Definition of the \texttt{WorkerStrategy} protocol interface for defining custom algorithms and logic to run on \worker{} nodes. }, 
    language=Python,
    label={lst:worker_strategy}, 
    float=t,
    boxpos=c,
    linewidth=0.985\columnwidth,
]
class WorkerStrategy(Protocol):
  def work_start(
    self, state: WorkerState
  ) -> WorkerState:
    pass
  def before_training(
    self, state: WorkerState, data: t.Any
  ) -> tuple[WorkerState, Any]:
    pass
  def after_training(
    self, state: WorkerState, opt: Optimizer
  ) -> WorkerState:
    pass
  def work_end(
    self, result: JobResult
  ) -> JobResult:
    pass
\end{lstlisting}

==> figures/comm_cost.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{graphics/plots/comm_cost_hier_vs_stand.pdf}
    \caption{Caption}
    \label{fig:enter-label}
\end{figure}

==> figures/tasks_per_sec.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{
        graphics/plots/tasks_per_sec_by_model.pdf
    }
    \caption{Throughput comparison between pure Parsl and Parsl with the RedisConnector (provided by Proxystore) for transferring increasingly large neural network models, ranging from 45MB to 231MB.}
    \label{fig:tasks_per_sec}
\end{figure}

==> figures/weak_scaling_flox.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{graphics/plots/end_prime_single.pdf}
    \caption{Weak scaling with \flox{}.}
    \label{fig:weak_scaling}
\end{figure}

==> tables/frameworks_old.tex <==
\begin{table}
\centering
\small
\caption{\flox{} compared with other FL frameworks.}
\begin{tabular}{rlll}
    \toprule
    Framework & DL Backend & Topology & Communication
    \\
    \midrule
    APPFL~\cite{appfl} & ? & 2-Tier & Agnostic
    \\
    Flower~\cite{flower} & Agnostic & 2-Tier & Agnostic
    \\
    FLoX~\cite{flox} & PyT, TF & 2-Tier & Globus Compute
    \\
    Substra~\cite{substra} & Agnostic & 2-Tier & -
    \\
    \flox{}~(ours) & PyTorch & 2-Tier, Hier. & Globus Compute
    \\
    \bottomrule
\end{tabular}
\end{table}
